Low-Subpacketization Multi-Antenna Coded Caching for Dynamic Networks

Multi-antenna coded caching combines a global caching gain, proportional to the total cache size in the network, with an additional spatial multiplexing gain that stems from multiple transmitting antennas. However, classic centralized coded caching schemes are not suitable for dynamic networks as they require prior knowledge of the number of users to indicate what data should be cached at each user during the placement phase. On the other hand, fully decentralized schemes provide comparable gains to their centralized counterparts only when the number of users is very large. In this paper, we propose a novel multi-antenna coded caching scheme for dynamic networks, where instead of defining individual cache contents, we associate users with a limited set of predefined caching profiles. Then, during the delivery phase, we aim at achieving a combined caching and spatial multiplexing gain, comparable to a large extent with the ideal case of fully centralized schemes. The resulting scheme imposes small subpacketization and beamforming overheads, is robust under dynamic network conditions, and incurs small finite-SNR performance loss compared with centralized schemes.

==> Data/L12.tex <==
SNR-dB	A5	A6	A7	B3	B4	B5	B6	B7	C2	C3	C4	C5	C6	C7	C8	C9	C10	NoCC	D5	D7	D8	D9	D10
0	6.405263305	6.558767841	6.447204769	5.698466288	5.987905377	6.138723755	6.291290118	6.378023876	0	5.508828933	5.68131052	5.842557541	6.012005324	6.233111045	6.147753539	6.247269058	6.259636818	4.9641	5.595330926	6.180064999	6.208950663	6.378255245	6.292827556
5	12.30358393	12.71700767	12.60675239	10.49983587	11.18956585	11.65566682	11.89608116	12.40200434	0	10.12897888	10.62521315	10.98354088	11.35991181	11.82433148	11.71926664	11.91537304	11.88997391	8.9824	10.40207605	11.68480779	11.80023492	12.06718186	12.00510619
10	20.37656607	21.35299471	21.34444308	16.84214433	18.12277221	19.10736393	19.46794216	20.89145031	0	16.32353439	17.33756384	18.01202037	18.68254814	19.4801821	19.33452412	19.64533094	19.57543415	14.2656	16.85962731	19.14816586	19.41704673	19.85492135	19.81983732
15	30.69026465	32.4836399	32.44715187	24.80104721	26.87612282	28.39933475	28.87888815	31.67118708	0	24.18507558	25.851178	27.00281427	28.01936967	29.15069296	28.95310898	29.32548521	29.2579388	20.9402	25.0416812	28.54736192	29.04668284	29.72597711	29.67077138
20	43.49195954	45.74183504	45.19847293	34.5979593	37.68538079	39.41852718	39.80783711	44.19579102	0	33.74650433	36.09160418	37.88626171	39.25874251	40.62958894	40.4398537	40.8040024	40.68816696	29.1397	34.99057488	39.77019283	40.58296087	41.49731296	41.38669277
25	58.50265025	60.27613297	58.75794351	45.94656457	50.23912592	51.68673213	51.61960292	57.69853388	0	44.58150376	47.58938551	50.10546522	51.81515447	53.35726423	53.25141142	53.55018195	53.25395658	38.5409	46.27704097	52.29987046	53.49566302	54.55556392	54.3820607
30	74.86727133	75.36270161	72.61983978	58.15785639	63.77884419	64.56786703	63.76370854	71.61104218	0	56.08041525	59.73257886	62.9729221	65.01340786	66.72536562	66.73110729	66.9130345	66.34238066	48.5774	58.2638454	65.49596152	67.1185543	68.22252209	67.98136526


==> Data/L15.tex <==
SNR-dB	A5	A6	A7	B3	B4	B5	B6	B7	C2	C3	C4	C5	C6	C7	C8	C9	C10	NoCC	D5	D7	D8	D9	D10
0	7.865162267	7.827670506	8.039871534	6.814589467	7.238732192	7.428305688	7.503559853	7.82200514	0	6.764882173	6.96054472	7.177410571	7.402219012	7.500626953	7.583867288	7.597378347	7.543599503	6.199972208	6.97045814	0	0	7.710681311	7.669187176
5	15.10384489	15.13565951	15.47788719	12.64800453	13.60554458	13.98449775	14.13434829	15.00819063	0	12.48946091	12.96688339	13.46319275	13.95515152	14.22362209	14.39079313	14.40579423	14.27789276	11.27518633	12.92543625	0	0	14.61025202	14.58249423
10	25.27301	25.41655773	25.73716886	20.65784356	22.42028868	22.91771272	23.07884979	24.9484851	0	20.30888194	21.19540707	22.11727433	22.98094641	23.50539851	23.75955003	23.76444992	23.51999975	18.14190161	21.0659554	0	0	24.11935695	24.10310574
15	38.34259129	38.21891728	38.05813056	30.74167215	33.56358853	33.88640579	33.81710796	37.04973136	0	30.01987618	31.41101944	32.89157883	34.15491363	34.95555651	35.2856819	35.24380728	34.81098696	26.65220242	31.17668057	0	0	35.82862378	35.7900695
20	53.67472791	52.55634617	51.43797062	42.3134097	46.38376203	46.16647067	45.55151512	50.37752848	0	40.97997146	42.94662339	45.07673493	46.7123742	47.75930911	48.16398484	48.02312175	47.32285341	36.2532966	42.59924683	0	0	48.88741066	48.79411551
25	70.22184359	67.56441564	65.22865108	54.62256692	60.03864902	59.02388317	57.64384905	64.21661881	0	52.51817601	55.09870328	57.92195064	59.90259611	61.16784104	61.64954652	61.37392221	60.36107988	46.35564825	54.63306727	0	0	62.53519259	62.36736372
30	87.2549295	82.81076387	79.15611025	67.21030798	74.01030119	72.05900884	69.8011886	78.22955065	0	64.26660624	67.4747866	71.00665503	73.31983709	74.79029903	75.35000701	74.9238151	73.58188298	56.63924008	66.88825672	0	0	76.38778837	76.13436668

